On the Effectiveness of Knowledge Graph Embeddings: a Rule Mining Approach

We study the effectiveness of Knowledge Graph Embeddings (KGE) for knowledge graph (KG) completion with rule mining. More specifically, we mine rules from KGs before and after they have been completed by a KGE to compare possible differences in the rules extracted. We apply this method to classical KGEs approaches, in particular, TransE, DistMult and ComplEx. Our experiments indicate that there can be huge differences between the extracted rules, depending on the KGE approach for KG completion. In particular, after the TransE completion, several spurious rules were extracted.

==> CEURART-DL/Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)

%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	# qpdf --linearize --newline-before-endstream $@ /tmp/$@
	# mv /tmp/$@ $@

unminted:
	@./minted2listings "*+minted.tex"

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto


==> tab_nrules_family.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
Model           & \multicolumn{1}{c}{Found} & \multicolumn{1}{c}{Missed} & \multicolumn{1}{c}{New} \\ \midrule
Random Baseline & 85                        & 9                          & 0                       \\
TransE          & 94                        & 0                          & 986                     \\
DistMult        & 93                        & 1                          & 90                      \\
ComplEx         & 94                        & 0                          & 43                      \\ \bottomrule
\end{tabular}%
\caption{\label{tab_nrules_family}Distribution of rules over the extended family KG, not counting duplicate rules that were mined from multiple extensions}
\end{table}


==> tab_nrules_wn18rr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htp]
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
Model           & \multicolumn{1}{c}{Found} & \multicolumn{1}{c}{Missed} & \multicolumn{1}{c}{New} \\ \midrule
Random Baseline & 9                         & 1                          & 0                       \\
TransE          & 10                        & 0                          & 707                     \\
DistMult        & 10                        & 1                          & 15                      \\
ComplEx         & 10                        & 0                          & 9                       \\ \bottomrule
\end{tabular}
\caption{\label{tab_nrules_wn18rr}Distribution of rules over the extended WN18RR KG, not counting duplicate rules that were mined from multiple extensions}
\end{table}


==> tab_overlap.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htb]
\centering
\begin{tabular}{@{}lrr@{}}
\toprule
Group (exclusive)                    & \multicolumn{1}{c}{WN18RR KG} & \multicolumn{1}{c}{Family KG} \\ \midrule
TransE                               & 693                           & 880                           \\
DistMult                             & 8                             & 3                             \\
ComplEx $\cap$ TransE                & 7                             & 19                            \\
DistMult $\cap$ TransE               & 5                             & 63                            \\
DistMult $\cap$ ComplEx$\cap$ TransE & 2                             & 24                            \\ \bottomrule
\end{tabular}
\caption{\label{tab:overlap}Count of rules found by extension group.  The groups are exclusive, meaning that ``ComplEx $\cap$ TransE'' only considers rules mined from both ComplEx and TransE-extended KGs but that were never mined from KGs extended with DistMult, for example.}
\end{table}

